AI, Pluralism, and (Social) Compensation

One strategy in response to pluralistic values in a user population is to personalize an AI system: if the AI can adapt to the specific values of each individual, then we can potentially avoid many of the challenges of pluralism. Unfortunately, this approach creates a significant ethical issue: if there is an external measure of success for the human-AI team, then the adaptive AI system may develop strategies (sometimes deceptive) to compensate for its human teammate. This phenomenon can be viewed as a form of social compensation, where the AI makes decisions based not on predefined goals but on its human partner's deficiencies in relation to the team's performance objectives. We provide a practical ethical analysis of the conditions in which such compensation may nonetheless be justifiable.

==> Solutions.tex <==
We posit that in situations where the outcome of a user’s decisions directly affects the well-being of another human, there exists a conflict between decision-maker autonomy and benefits to others \cite{abramson1989autonomy}. Most discussions of human-algorithm interaction focus on situations in which the human knows better than the algorithm, and their decision affects them. However, numerous studies have demonstrated AI systems to be fairer and more impartial than their human counterparts \cite{sullivan2018employing, kleinberg2018human, bertrand2004emily, rizer2018artificial, wang2023biased}. These systems do not suffer the cognitive and moral biases that often influence human judgment and so can provide valuable insights for developing more equitable decision-making approaches. Of course, this performance depends on having training data that do not encode those human biases; certainly, many AI systems are as biased as humans, if not more so. There are many well-justified concerns about biases and errors from AI systems, but that fact should not lead us to overlook the potential impacts of human biases, particularly in high-stakes domains like criminal justice or healthcare.

For instance, a judge's use of AI to counteract personal biases in private matters is a personal choice. However, when judicial decisions affect defendants, the involvement of AI raises critical ethical and legal questions. This scenario unveils a paradox: an AI system designed to be ethically aware and pluralistic may produce recommendations that are fair to the defendant but challenge its human collaborator's inherent biases or immediate interests. A challenge lies in developing AI systems that can embrace diverse perspectives while effectively partnering with humans who possess individual biases and preferences. How can this technology support better decision-making? In situations where there is a reasonable expectation that the user's biases could lead to suboptimal or biased outcomes, what responsibilities do the developers\footnote{In this context, a \textbf{developer} refers to the individual or team responsible for creating, maintaining, and refining the algorithm to align with intended objectives and ethical standards.}  of these algorithms bear?  


Compensating for a user's bias might seem like a case of paternalism \cite{kleinig1983paternalism}, as it involves questioning whether the developer's value judgments should be imposed on the user. However, in many cases, the primary beneficiary of the developer’s actions is the decision 'target' rather than the algorithm user, which means the traditional framework of paternalism does not apply directly. Nonetheless, the line between paternalism and the proposed approach can be blurry, carrying a risk of overstepping boundaries. Therefore, developers must be cautious not to impose their value systems on users without considering user autonomy. The judicious mitigation of user bias is not to restrict free choice; rather, it is to guide it toward the higher rational principle of consequentialism \cite{mcelwee2010rights}. Similarly to how we accept reasonable limits on liberty to prevent violations of others' rights, we must recognize that unchecked risks can lead to significant ethical breaches if not moderated by a focus on outcomes. Therefore, it is not only acceptable but sometimes necessary for algorithm developers to take steps to compensate for user biases when there is a significant risk of harm to others. By doing so, developers can ensure that their algorithms are being used in a manner that aligns with the principles of non-maleficence and beneficence \cite{page2012four}. 



==> related.tex <==
\subsection{Decision-making in Human-AI Systems}
Various studies have shown that AI systems can be fairer and more impartial than their human counterparts \cite{sullivan2018employing, kleinberg2018human, bertrand2004emily, rizer2018artificial, wang2023biased}. AI systems do not suffer the cognitive and moral biases that often influence human judgment, and so can provide valuable insights for developing more equitable decision-making approaches. Of course, this performance depends on having training data that do not encode those human biases; certainly, many AI systems are as biased as humans, if not more so. There are many well-justified concerns about biases and errors from AI systems, but that fact should not lead us to overlook the potential impacts of human biases.

Theoretically, the combination of human expertise and AI should yield decision-making outcomes that surpass the individual capabilities of either entity. One barrier to this goal are human biases that are persistent, such as over-reliance on or mistrust of AI decisions \cite{lee2004trust,poursabzi2021manipulating}.  Even when AI systems are designed to counteract these biases, the subjective nature of human decisions can undermine overall effectiveness \cite{10.1145/3534561,rastogi}. This issue is further exacerbated by variations in user expertise and decision-making style.
Current research reveals significant gaps in understanding and mitigating biases within human-AI systems. Although many studies focus on scenarios where users are unaware of biases, they often overlook situations where direct nudges and training are ineffective because users recognize and resist the influence tactics \cite{sunstein2017nudges, hummel2019effective}. Additionally, users may be reluctant to make choices that benefit the broader good, leading to decisions affected by various biases, including cognitive and moral ones.% There is also a scarcity of research addressing the challenge of counteracting biases when users are disinclined to do so, despite the broader impact of their decisions.

\subsection{}

